A Collapse Theorem for Holographic Algorithms with Matchgates on Domain Size at Most 4

Holographic algorithms with matchgates are a novel approach to design polynomial time computation. It uses Kasteleyn's algorithm for perfect matchings, and more importantly a holographic reduction . The two fundamental parameters of a holographic reduction are the domain size $k$ of the underlying problem, and the basis size $\ell$. A holographic reduction transforms the computation to matchgates by a linear transformation that maps to (a tensor product space of) a linear space of dimension $2^{\ell}$. We prove a sharp basis collapse theorem, that shows that for domain size 3 and 4, all non-trivial holographic reductions have basis size $\ell$ collapse to 1 and 2 respectively. The main proof techniques are Matchgates Identities, and a Group Property of matchgates signatures.

==> d2.tex <==
\section{A New Proof for the Collapse Theorem os Domain Size 2}
In $\cite{string6}$, Cai and Lu has proved a collapse theorem for domain size 2. Here we give a new proof by MGI and group property of standard signatures.

In this section, assume that $G$ is a generator of full rank on domain size 2, the basis $M$ is a $2^{\ell}\times 2$ matrix and rank$(M)=2$, and $\underline{G}=M^{\otimes n}G$ is a standard signature of arity $n\ell$.
So there exists $t\in[n]$ such that rank$(G(t))=2$ and rank$(\underline{G}(t))=2$, where $\underline{G}(t)=MG(t)(M^{\tt{t}})^{\otimes (n-1)}$. Then we can define $\alpha_{\sigma}, \alpha_{\tau}, \beta_{\zeta}, \beta_{\eta}$ as follows:
\begin{itemize}
\item $\underline{G}(t)^{\alpha_{\sigma}}, \underline{G}(t)^{\alpha_{\tau}}$ are linearly independent,
\item ${\rm wt}(\alpha_{\sigma}+\alpha_{\tau})=\displaystyle\min_{\alpha_{u}\neq \alpha_{v}, \alpha_{u}, \alpha_{v}\in\{0, 1\}^{\ell}}\{{\rm wt}(\alpha_{u}+\alpha_{v})|\underline{G}(t)^{\alpha_{u}}, \underline{G}(t)^{\alpha_{v}}$
  are linearly independent $\}$.
\end{itemize}
Let $x_{\beta}=\begin{pmatrix}
\underline{G}^{\beta\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta\curvearrowleft_{t} \alpha_{\tau}}
\end{pmatrix}$, then there exist $\beta_{\zeta}, \beta_{\eta}$ such that:

\begin{itemize}
\item $x_{\beta_{\zeta}}, x_{\beta_{\eta}}$ are linearly independent,
\item ${\rm wt}(\beta_{\zeta}+\beta_{\eta})=\displaystyle\min_{\beta_{u}\neq \beta_{v}, \beta_{u}, \beta_{v}\in\{0, 1\}^{(n-1)\ell}}\{{\rm wt}(\beta_{u}+\beta_{v})|x_{\beta_{u}},x_{\beta_{v}}$ are linearly independent $\}$.
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
One can always
add an extra edge at an external node to flip the bit from 1 to 0 to ¡°move¡± 0 to the all 0 vector.

To simplify notations in
the following proof, we assume  $\alpha_{\sigma}$ (where there are a 1s, a is odd).
This simplifying assumption is without loss of generality; see the remarks after the proof.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Then we directly have the following lemma that is simple but very useful.
\begin{lemma}\label{lemma4.1.1}
If there exists $\alpha$ such that $0<{\rm wt}(\alpha+\alpha_{\sigma})<{\rm wt}(\alpha_{\sigma}+\alpha_{\tau})$ and
$0<{\rm wt}(\alpha+\alpha_{\tau})<{\rm wt}(\alpha_{\sigma}+\alpha_{\tau})$, then $\underline{G}(t)^{\alpha}$ is identical zero, i.e., all the entries of  $\underline{G}(t)^{\alpha}$  are 0. Similarly, If there exists $\beta$ such that $0<{\rm wt}(\beta+\beta_{\eta})<{\rm wt}(\alpha_{\eta}+\alpha_{\zeta})$ and
$0<{\rm wt}(\beta+\beta_{\zeta})<{\rm wt}(\beta_{\eta}+\beta_{\zeta})$, then $x_{\beta}$ is identical zero, i.e., all the entries of  $x_{\beta}$  are 0.
\end{lemma}

%\begin{remark}
%Let $\alpha_{\tau}=\alpha_{\sigma}+e_{p_{1}}+e_{p_{2}}+\cdots +e_{p_{d}}$,
% $\beta_{\eta}=\beta_{\zeta}+e_{q_{1}}+e_{q_{2}}+\cdots +e_{q_{d'}}$, then
 %$\underline{G}(t)^{\beta\curvearrowleft_{t}(\alpha_{\sigma}+e_{p_{i_{1}}}+e_{p_{i_{2}}}+\cdots +e_{p_{i_{s}}})}=0$,
% $\underline{G}(t)^{\beta\curvearrowleft_{t}(\alpha_{\tau}+e_{p_{i_{1}}}+e_{p_{i_{2}}}+\cdots +e_{p_{i_{s}}})}=0$, where
% $\beta\in\{0,1\}^{(n-1)\ell}$, $s< d$ and $p_{i_{1}}, p_{i_{2}}, \cdots, p_{i_{s}}\in\{p_{1}, p_{2}, \cdots, p_{d}\}$.
%Furthermore, $\underline{G}(t)^{(\beta_{\zeta}+e_{q_{i_{1}}}+e_{q_{i_{2}}}+\cdots +e_{q_{i_{s'}}})\curvearrowleft_{t}\alpha_{\sigma}}=0$,
%$\underline{G}(t)^{(\beta_{\eta}+e_{q_{i_{1}}}+e_{q_{i_{2}}}+\cdots +e_{q_{i_{s'}}})\curvearrowleft_{t}\alpha_{\sigma}}=0$,
%\newline
%$\underline{G}(t)^{(\beta_{\zeta}+e_{q_{i_{1}}}+e_{q_{i_{2}}}+\cdots +e_{q_{i_{s'}}})\curvearrowleft_{t}\alpha_{\tau}}=0$,
%$\underline{G}(t)^{(\beta_{\eta}+e_{q_{i_{1}}}+e_{q_{i_{2}}}+\cdots +e_{q_{i_{s'}}})\curvearrowleft_{t}\alpha_{\tau}}=0$,
%where
%$s'< d'$ and $q_{i_{1}}, q_{i_{2}}, \cdots, q_{i_{s'}}\in\{q_{1}, q_{2}, \cdots, q_{d'}\}$.
%\end{remark}

%\begin{lemma}$^{\cite{string6}}$
%\label{lemma4.1}
%If $G$ is a generator of full rank and $\underline{G}=M^{\otimes n}G$, then any two rows of same parity of $M$ are linearly dependent respectively.
%\end{lemma}


\begin{lemma}
\label{lemma4.2}
Let $d={\rm wt}(\alpha_{\sigma}+\alpha_{\tau})$,
  then $d=1$.
\end{lemma}
\begin{proof}
%Firstly, from
%\begin{center}
%$\begin{pmatrix}
%\underline{G}(t)^{\alpha_{\sigma}}\\
%\underline{G}(t)^{\alpha_{\tau}}
%\end{pmatrix}=
%\begin{pmatrix}
%M^{\alpha_{\sigma}}\\
%M^{\alpha_{\tau}}
%\end{pmatrix}
%G(t)(M^{\textbf{t}})^{\otimes (n-1)},
%$
%\end{center}
%we have
%rank$\begin{pmatrix}
%M^{\alpha_{\sigma}}\\
%M^{\alpha_{\tau}}
%\end{pmatrix}=2$, so $d\neq 2$ from Lemma \ref{lemma4.1}.
%%%%%%%%%%%%%%

Assume that $d\geq 2$.  Let $x_{\beta_{\zeta}}=\begin{pmatrix}
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}
\end{pmatrix}$,
$x_{\beta_{\eta}}=\begin{pmatrix}
\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\tau}}
\end{pmatrix}$
and
%Secondly, if there exists $\alpha$ that has the same parity to $\alpha_{\sigma}, \alpha_{\tau}$ such that $0< d(\alpha,\alpha_{\sigma})< d(\alpha_{\sigma},\alpha_{\tau})$ and $0< d(\alpha,\alpha_{\tau})< d(\alpha_{\sigma},\alpha_{\tau})$,
%then $\underline{G}_{i}^{\alpha}$ is a 0 vector by the definition of $d(\alpha_{\sigma},\alpha_{\tau})$. Similarly,
%if there exists $\beta$ such that $0< d(\beta,\beta_{\zeta})< d(\beta_{\zeta},\beta_{\eta})$ and $0< d(\beta,\beta_{\eta})< d(\beta_{\zeta},\beta_{\eta})$, then
%$x_{\beta}$ is 0 vector by the definition of $d(\beta_{\zeta},\beta_{\eta})$.
%
 $\alpha_{\tau}=\alpha_{\sigma}+e_{p_{1}}+e_{p_{2}}+\cdots +e_{p_{d}}$,
 $\beta_{\eta}=\beta_{\zeta}+e_{q_{1}}+e_{q_{2}}+\cdots +e_{q_{d'}}$. We will prove $\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\tau}}-
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}=0$ by MGI to get a contradiction.

Let the position be $(q_{1}q_{2}\cdots q_{d'})\curvearrowleft_{t}(\bar{p}_{1}\bar{p}_{2}\cdots \bar{p}_{d})$  and
the pattern be $\beta_{\zeta}\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}})$ and $\beta_{\zeta}\curvearrowleft_{t} (\alpha_{\tau}
+e_{\bar{p}_{1}})$ respectively,
from MGI, we have

\begin{equation}\label{MGI4.1}
\displaystyle\sum_{u=1}^{d}(-1)^{u+1}\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}}+e_{\bar{p}_{u}})}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} (\alpha_{\tau}
+e_{\bar{p}_{1}}+e_{\bar{p}_{u}})}=
\displaystyle\sum_{v=1}^{d'}(-1)^{f(v)}\underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}})}\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\tau}+e_{\bar{p}_{1}})},
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}\label{MGI4.2}
\displaystyle\sum_{u=1}^{d}(-1)^{u+1}\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} (\alpha_{\tau}
+e_{\bar{p}_{1}}+e_{\bar{p}_{u}})}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}}+e_{\bar{p}_{u}})}=
\displaystyle\sum_{v=1}^{d'}(-1)^{f(v)}\underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\tau}+e_{\bar{p}_{1}})}\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}})},
\end{equation}
where $f(v)$ is 0 or 1.

If $d=2$, from (\ref{MGI4.1}), we have
\begin{center}
$\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\tau}}-
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}=\displaystyle\sum_{v=1}^{d'}(-1)^{f(v)}\underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}})}\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\tau}+e_{\bar{p}_{1}})}$.
\end{center}
$\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\tau}+e_{\bar{p}_{1}})}=0$ for $1\leq v\leq d'$ from Lemma \ref{lemma4.1.1},
so $\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\underline{G}^{\beta_{\eta}
\curvearrowleft_{t} \alpha_{\tau}}-\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}=0$.
This contradicts that
$x_{\beta_{\zeta}}=\begin{pmatrix}
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}
\end{pmatrix}$,
$x_{\beta_{\eta}}=\begin{pmatrix}
\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta_{\eta}
\curvearrowleft \alpha_{\tau}}
\end{pmatrix}$
are linearly independent, so $d\neq 2$.


If $d>2$, then $\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}}+e_{\bar{p}_{u}})}=0$
 for $u>1$ from Lemma \ref{lemma4.1.1} and $d>2$. From (\ref{MGI4.1}), (\ref{MGI4.2}), we have
\begin{equation}\label{MGI4.3}
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\underline{G}^{\beta_{\eta}
\curvearrowleft_{t} \alpha_{\tau}}=
\displaystyle\sum_{v=1}^{d'}(-1)^{f(v)}\underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}})}\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\tau}+e_{\bar{p}_{1}})},
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{equation}\label{MGI4.4}
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}=
\displaystyle\sum_{v=1}^{d'}(-1)^{f(v)}\underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\tau}+e_{\bar{p}_{1}})}\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}})}.
\end{equation}
In the right hand of (\ref{MGI4.3}), (\ref{MGI4.4}),
$\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\tau}+e_{\bar{p}_{1}})}=0,$
$\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t} (\alpha_{\sigma}+e_{\bar{p}_{1}})}=0$ for $1\leq v\leq d'$ from Lemma \ref{lemma4.1.1},
so $\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\underline{G}^{\beta_{\eta}
\curvearrowleft_{t} \alpha_{\tau}}=0$,
$\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}=0$.
This contradicts that
$x_{\beta_{\zeta}}=\begin{pmatrix}
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}
\end{pmatrix}$,
$x_{\beta_{\eta}}=\begin{pmatrix}
\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta_{\eta}
\curvearrowleft \alpha_{\tau}}
\end{pmatrix}$
are linearly independent, so $d=1$.
\end{proof}
In the following discussion, let $\alpha_{\tau}=\alpha_{\sigma}+e_{p_{1}}$.
\begin{lemma}
  \label{lemma4.4}
  Let $d'={\rm wt}(\beta_{\zeta}+\beta_{\eta})$, then $d'=1$.
  \end{lemma}
\begin{proof}
 Assume that $d'>1$ and $\beta_{\eta}+\beta_{\zeta}=e_{q_{1}}+e_{q_{2}}+\cdots +e_{q_{d'}}$.
Let
the position be $(q_{1}q_{2}\cdots q_{d'})\curvearrowleft_{t} \bar{p}_{1}$
and the pattern be $\beta_{\zeta}\curvearrowleft_{t}(\alpha_{\sigma}+e_{\bar{p}_{1}})$
and $\beta_{\zeta}\curvearrowleft_{t}(\alpha_{\tau}+e_{p_{1}})$ respectively, then from MGI
\begin{equation}
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t}\alpha_{\sigma}}\underline{G}^{\beta_{\eta}
\curvearrowleft_{t}\alpha_{\tau}}=
\displaystyle\sum_{v=1}^{d'}(-1)^{f(v)}\underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t}\alpha_{\tau}}
\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t}\alpha_{\sigma}},
\end{equation}
\begin{equation}
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t}\alpha_{\tau}}\underline{G}^{\beta_{\eta}
\curvearrowleft_{t}\alpha_{\sigma}}=
\displaystyle\sum_{v=1}^{d'}(-1)^{f(v)}\underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t}\alpha_{\sigma}}
\underline{G}^{(\beta_{\eta}+e_{q_{v}})\curvearrowleft_{t}\alpha_{\tau}},
\end{equation}
where $f(v)$ is 0 or 1.

%Note that if there exists $\beta$ such that $0< {\rm wt}(\beta+\beta_{\zeta})< {\rm wt}(\beta_{\eta}+\beta_{\zeta})$
%and $0< {\rm wt}(\beta+\beta_{2})<{\rm wt}(\beta_{\eta}+\beta_{\zeta})$,
%then all entries of $x_{\beta}$ are 0, so

By Lemma
\ref{lemma4.1.1}
$\underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t}\alpha_{\tau}}=0, \underline{G}^{(\beta_{\zeta}+e_{q_{v}})\curvearrowleft_{t}\alpha_{\sigma}}=0$
 for $1\leq v\leq d'$,
so $\underline{G}^{\beta_{\zeta}\curvearrowleft_{t}\alpha_{\sigma}}\underline{G}^{\beta_{\eta}
\curvearrowleft_{t}\alpha_{\tau}}=0$,
$\underline{G}^{\beta_{\zeta}\curvearrowleft_{t}\alpha_{\tau}}\underline{G}^{\beta_{\eta}\curvearrowleft_{t}\alpha_{\sigma}}=0$.
This contradicts that $x_{\beta_{\zeta}}=\begin{pmatrix}
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\tau}}
\end{pmatrix}$,
$x_{\beta_{\eta}
}=\begin{pmatrix}
\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\sigma}}\\
\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\tau}}
\end{pmatrix}$
are linearly independent.
So $d'=1$.
\end{proof}

%If the rows $M^{\alpha_{\sigma}}, M^{\alpha_{\tau}}$ in $M$ are linearly dependent, then $\underline{G}(t)^{\alpha_{\sigma}}, \underline{G}(t)^{\alpha_{\tau}}$
%are linearly dependent. So
In the following discussion, let $\beta_{\eta}=\beta_{\zeta}+e_{q_{1}}$.

\begin{lemma}
\label{lemma4.3}
$\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}=(M^{\alpha_{\sigma}, \alpha_{\tau}})^{\otimes n}G$ is a standard signature of arity $n$.
\end{lemma}
\begin{proof}
Let $\Gamma$ be the matchgate realizing $\underline{G}$. Carry out the following transformations of $\Gamma$ to get a new matchgate $\Gamma'$:
For every block of $\Gamma$, if the $i-th$ bit of $\alpha_{\sigma}$ is 0, do nothing to it.
If the $i-th$ bit of $\alpha_{\sigma}$ is 1, we connect an edge with weight 1 to the $((j-1)\ell+i)-th$ node
 for $1\leq i\leq\ell, 1\leq j\leq n$.
 %and $i\neq p_{1}$.

 Note that all of the bits of $\alpha_{\sigma}, \alpha_{\tau}$
are same except for the $p_{1}-th$ bit.
View
 the $((j-1)\ell+p_{1})$-th node of $\Gamma'$ as external nodes for $1\leq j\leq n$ and all other nodes as internal nodes,
 then its standard signature is $\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}.$
 \end{proof}

 \begin{remark}
 Note that $\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}$ is a standard signature of arity $n$. Denoted it as
 $\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}=(\underline{\check{G}}^{i_{1}i_{2}\cdots i_{n}})$, then
 $\underline{\check{G}}^{i_{1}i_{2}\cdots i_{n}}$ is an entry of $\underline{G}$ and its index in $\underline{G}$ is
 $\alpha_{1}\alpha_{2}\cdots \alpha_{n}$, where $\alpha_{s}\in \{\alpha_{\sigma}, \alpha_{\tau}\}$ and $i_{s}=0$ if
 $\alpha_{s}=\alpha_{\sigma},$ $ i_{s}=1$  if
 $\alpha_{s}=\alpha_{\tau}$ for $1\leq s\leq n$. \end{remark}


  From Lemma \ref{lemma4.2}, \ref{lemma4.4}, \ref{lemma4.3}, we have
\begin{coro}  Let $\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}=(\underline{\check{G}}^{i_{1}i_{2}\cdots i_{n}})$,
then  there exists $\beta\in\{0,1\}^{(n-1)}, q_{1}$ such that $\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}(t)_{\beta,\beta+e_{q_{1}}}$ has full rank.
\end{coro}

\begin{coro}
$\begin{pmatrix}
M^{\alpha_{\sigma}}\\
M^{\alpha_{\tau}}
\end{pmatrix}$
has rank 2.
since
$\begin{pmatrix}
\underline{G}(t)^{\alpha_{\sigma}}\\
\underline{G}(t)^{\alpha_{\tau}}
\end{pmatrix}=
\begin{pmatrix}
M^{\alpha_{\sigma}}\\
M^{\alpha_{\tau}}
\end{pmatrix}
G(t)(M^{\tt{T}})^{\otimes (n-1)}.$
\end{coro} 
 \begin{lemma}
 \label{standard recognizer for d2}
 There exists  a standard signature $\underline{R}$ of a recognizer matchgate of airty $n$ such that $\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}(t)\underline{R}(t)=I_{2}$, where
 $\underline{R}(t)$ is the $t-th$ matrix form of $\underline{R}$ as a recognizer.
 \end{lemma}

\begin{proof}
W. l. o. g.,
assume that  $\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}$ has a full rank sub-matrix of the form
$\begin{pmatrix}
\underline{G}^{\beta_{\zeta}
\curvearrowleft_{t} \alpha_{\sigma}}&0\\
0&\underline{G}^{\beta_{\eta}
\curvearrowleft_{t} \alpha_{\tau}}
\end{pmatrix}.$
%(The proof of the following lemma if the sub-matrix of the form $\begin{pmatrix}
%0&\underline{G}^{\beta_{\eta}\curvearrowleft \alpha_{\sigma}}\\
%\underline{G}^{\beta_{\zeta}
%\curvearrowleft \alpha_{\tau}}&0
%\end{pmatrix}$ is similar, so we omit it).
Let $i_{1}\cdots i_{t-1}0 i_{t+1}\cdots i_{n}$ and $j_{1}\cdots j_{t-1}1 j_{t+1}\cdots j_{n}$ be the corresponding index of
$\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}$, $\beta_{\eta}\curvearrowleft_{t} \alpha_{\tau}$ in $\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}$ respectively. Note that ${\rm wt}(i_{1}\cdots i_{t-1}0 i_{t+1}\cdots i_{n}+j_{1}\cdots j_{t-1}1 j_{t+1}\cdots j_{n})=2$.
Let $\underline{R}=(\underline{R}^{i_{1}i_{2}\cdots i_{n}})$ be a row vector of dimension $2^{n}$, where
$\underline{R}^{i_{1}\cdots i_{t-1}0 i_{t+1}\cdots i_{n}}=(\underline{G}^{\beta_{\zeta}\curvearrowleft_{t} \alpha_{\sigma}})^{-1}$,
$\underline{R}^{j_{1}\cdots j_{t-1}1 j_{t+1}\cdots j_{n}}=(\underline{G}^{\beta_{\eta}\curvearrowleft_{t} \alpha_{\tau}})^{-1}$, and all other entries are 0,
then
$\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}(t)\underline{R}(t)
=I_{2}$,  where $\underline{R}(t)$ is the $t-th$
matrix form of $\underline{R}$ as a recognizer.
Furthermore, there are only two non-zero entries in $\underline{R}$ and the Hamming distance of their index is 2, so $\underline{R}$
satisfies the parity constrains and MGI. By Lemma \ref{MGI}, there is a matchgate $\Gamma_{0}$ realizing $\underline{R}$.
\end{proof}


\begin{lemma}
\label{lemma4.5}
Assume that $G$ is a generator of full rank, $\underline{G}=M^{\otimes n}G$ and $T=M(M^{\alpha_{\sigma}, \alpha_{\tau}})^{-1}$, then $T$ is a transformer
of $\ell-$ output and 1-input.
\end{lemma}
\begin{proof}
Note that $T^{\alpha_{\sigma}, \alpha_{\tau}}=I_{2}$ and
$\underline{G}=M^{\otimes n}G=T^{\otimes n}(M^{\alpha_{\sigma}, \alpha_{\tau}})^{\otimes n}G=T^{\otimes n}\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}$, so
\begin{center}
$\underline{G}^{t^{c}\leftarrow\alpha_{\sigma}, \alpha_{\tau}}(t)=
 T\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}(t)(T^{\alpha_{\sigma}, \alpha_{\tau}})^{\tt{T} \otimes n-1}
 =T\underline{G}^{*\leftarrow\alpha_{\sigma}, \alpha_{\tau}}(t)$.
 \end{center}

 Let $\underline{R}$, $\Gamma_{0}$ be defined as Lemma \ref{standard recognizer for d2} and $\Gamma$ be the matchgate realizing
 $\underline{G}$. Carry out the same transformations to
 $i-th$ block of $\Gamma$ for $1\leq i\leq n, i\neq t$ as Lemma \ref{lemma4.3}, then we get a new matchgate $\Gamma''$ of $n\ell$ output nodes
 $Y_{1,1}, Y_{1,2}, \cdots, Y_{1,\ell}, Y_{2,1}, Y_{2,2}, \cdots, Y_{2,\ell}, \cdots, Y_{n, 1}, Y_{n, 2}, \cdots, Y_{n,\ell}.$

 Let the input nodes of
 $\Gamma_{0}$ be $X_{1}, X_{2},\cdots, X_{n}$ and
 join the node $Y_{(i-1)\ell, p_{1}}$ of $\Gamma''$ and  $X_{i}$ with an edge of weight 1 for $1\leq i\leq n$ and $i\neq t$,
 then we get a transformer matchgate with $Y_{t,1}, Y_{t,2},\cdots, Y_{t,\ell}$ as output nodes, $X_{t}$ as input nodes, and its standard signature is
$T=\underline{G}^{t^{c}\leftarrow\alpha_{\sigma}, \alpha_{\tau}}(t)\underline{R}(t)$.
\end{proof}
We illustrate Lemma \ref{lemma4.5} by the Fig 1 in the Appendix.

\begin{theorem}
Any holographic algorithm on a basis of size $\ell$ and domain size 2 which employs at least one generator of full rank can be simulated
on a basis of size 1.
\end{theorem}
\begin{proof}
 If $\underline{R}_{i}M^{\otimes n}=R_{i}$ for $1\leq i\leq r$ and $\underline{G}_{j}=M^{\otimes n}G_{j}$ for $1\leq j\leq g$, where $R_{i}, G_{j}$
 are recognizers and generators that a holographic algorithm employs and $\underline{R}_{i}, \underline{G}_{j}$ are standard signatures,
 then $\underline{R}'_{i}(M^{\alpha_{\sigma}, \alpha_{\tau}})^{\otimes n}=R_{i}$ for $1\leq i\leq r$ and $\underline{G}_{j}^{*\leftarrow \alpha_{\sigma}, \alpha_{\tau}}=(M^{\alpha_{\sigma}, \alpha_{\tau}})^{\otimes n}G_{j}$ for $1\leq j\leq g$,
 where $\underline{R}_{i}'=\underline{R}_{i}T^{\otimes n}$, $\underline{G}_{j}^{*\leftarrow \alpha_{\sigma}, \alpha_{\tau}}$  are standard signatures by Lemma \ref{product transformer}, Lemma \ref{lemma4.3} . This implies that $R_{i}, G_{j}$ are simultaneously realized on the basis $M^{\alpha_{\sigma}, \alpha_{\tau}}$.
\end{proof} 

